Hamster: A Large-Scale Study and Characterization of Developer-Written Tests

Automated test generation (ATG), which aims to reduce the cost of manual test suite development, has been investigated for decades and has produced countless techniques based on a variety of approaches: symbolic analysis, search-based, random and adaptive-random, learning-based, and, most recently, large-language-model-based approaches. However, despite this large body of research, there is still a gap in our understanding of the characteristics of developer-written tests and, consequently, our assessment of how well ATG techniques and tools can generate realistic and representative tests. To bridge this gap, we conducted an extensive empirical study of developer-written tests for Java applications, covering 1.7 million test cases from open-source repositories. Our study is the first of its kind to evaluate aspects of developer-written tests that are mostly neglected in the existing literature -- including test scope, test fixtures and assertions, types of inputs, and use of mocking -- and characterize tests accordingly. Based on this characterization, we then compare existing tests with those generated by two state-of-the-art ATG tools. Our results highlight that the vast majority of developer-written tests exhibit characteristics that are beyond the capabilities of current ATG tools. Finally, based on our findings, we identify promising research directions that can help develop more effective tool support for developer testing practices. We believe this work can set the stage for additional research and bring ATG tools closer to generating the types of tests developers write.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
% Here, we discuss the key findings and the next steps for the research community.

% \vskip 2pt
\noindent\textit{Complex test generation.}
Developer-written tests often exceed targeting a single focal class or method; instead, they span multiple classes to validate higher-level behaviors. These tests tend to be more complex and are currently beyond the capabilities of most ATG tools. This presents a promising research direction---developing techniques to generate tests for more intricate scenarios. 

\vskip 1pt
\noindent\textit{Modular and reusable test suites.}
A prominent pattern in developer-written tests is the emphasis on modularity and reuse---achieved through the use of test fixtures, helper methods, and repeated call–assertion blocks. These design choices enhance maintainability and make the tests more intuitive to developers. This is another opportunity for the research community to explore modular test design and build ATG tools that not only generate tests with high code coverage, but do so in a modular and maintainable manner. % aligned with real-world testing practices.

\vskip 1pt
\noindent\textit{Complex call and assertion sequences.}
Developer-written tests often incorporate complex patterns such as grouped assertions, assertion chaining, etc. These patterns enhance test expressiveness, and could be effectively leveraged by future ATG tools. LLMs, in particular, are well-positioned to capture these behaviors due to their inherent exposure to developer-written codebases. However, targeted research is needed to develop techniques that can reliably surface and apply such patterns during test generation---especially while maintaining high code coverage and test quality.

\vskip 1pt
\noindent\textit{Complex inputs.} Another research direction is supporting complex test inputs, which are often required when tests interact with databases, external services, or structured data formats (e.g., JSON, XML, CSV). Developing techniques to infer data schemas and ensure self-contained test execution could be a direction to explore.

==> table/match.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table}
  \centering
  \caption{Matching call-assertion sequences.}
  \setlength{\tabcolsep}{3pt}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|r|c|c|c|c|c}
    \toprule
    \multicolumn{1}{c|}{Match ($M$)} & \multicolumn{1}{c|}{CA} & $M=100$\%  & $100\%>M\geq70$\% & $70\%>M\geq50\%$ & $50\%>M\geq30\%$ & $M<30\%$ \\
    \midrule
    OD & \multirow{2}{*}{3,654,835} & 39.7\%    &   1.7\%    &    6.3\%   &    2.4\%   &     49.8\%   \\
    OID &       & 40.5\% & 5.3\% & 11.5\% & 5.7\% & 37.0\% \\
    \bottomrule
    \end{tabular}%\\
    }
    \scriptsize\\
    * CA: Number of call-assertion sequences, OD: Order dependent, OID: Order independent
  \label{tb:match}%
  \vspace{-5pt}
\end{table}%


==> table/test_method.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Test method characteristics.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \textbf{Metrics} & \multicolumn{4}{c|}{\textbf{UI Test}}   & \multicolumn{4}{c|}{\textbf{API Test}}  & \multicolumn{4}{c|}{\textbf{Library Test}} &  \multicolumn{8}{c}{\textbf{Rest of the tests}}\\
    \cline{14-21}
     & \multicolumn{4}{c|}{\textbf{}}   & \multicolumn{4}{c|}{\textbf{}}  & \multicolumn{4}{c|}{\textbf{}} & \multicolumn{4}{c|}{\textbf{1 focal class}} & \multicolumn{4}{c}{\textbf{>1 focal class}}\\
    \hline
    Total tests & \multicolumn{4}{c|}{9596}          & \multicolumn{4}{c|}{}          & \multicolumn{4}{c|}{}          & \multicolumn{4}{c|}{}& \multicolumn{4}{c}{} \\
    \hline
    \hline
    Percentile & \textbf{P25}   & \textbf{P50}   & \textbf{P75}   & \textbf{P90}   & \textbf{P25}   & \textbf{P50}   & \textbf{P75}   & \textbf{P90}   & \textbf{P25}   & \textbf{P50}   & \textbf{P75}   & \textbf{P90}   & \textbf{P25}   & \textbf{P50}   & \textbf{P75}   & \textbf{P90} & \textbf{P25}   & \textbf{P50}   & \textbf{P75}   & \textbf{P90} \\
    \hline
    \hline
    NCLOC &   6    &   8    &  13     &   19    &    8   &   12    &   18    &    28   &   3    &   6    &   11    &  19     &    5   &    8   &   14    & 23 & 7& 12& 22& 37  \\
    \hline
    \# of objects created &    0   &    0   &   3    &    6   &    0   &    0   &    3   &    6   &    0   &   0    &   1    &   4    &    0   &   1    &   3    & 7 & 0 & 2& 6& 12 \\
    \hline
    \# of mocks &    1   &    2   &    3   &    4   &   1    &     1  &   2    &    4   &   1    &  1     &   3    &  5     &    1   &   2    &    3   & 6 & 1& 2&4 &8 \\
    \hline
    \# of constructor calls &   0    &     0  &    3   &   6    &   0    &    0   &   3    &    6   &   0    &   0    &   1    &   4    &    0   &   1    &  3     & 7 & 0& 2 &6 & 12\\
    \hline
    \# of application calls &   1    &   3    &    7   &   12    &    1   &    2   &   6    &     12  &   0    &     0  &    1   &    3   &    1   &  2     &   5    &  10 &3 & 6& 13& 25\\
    \hline
    \# of library calls &    0   &   2    &    7   &   15    &    4   &   9    &   14    &     24  &     1  &    1   &   2    &    6   &    0   &    1   &   4    &  9 & 1& 3& 8& 16\\
    \hline
    \# of call-assertion sequence &    1   &     2  &   3    &     4  &  1     &     1  &   1    &   3    &   1    &    1   &   2    &   3    &   1    &   1    &  2     & 5 & 1& 2& 4& 7\\
    \hline
    \# of calls &   5    &  8     &   15    &    24   &    10   &  16     &  24     &  39     &  1     &   3    &    8   &   15    &    3   &    16   &   13    & 23 &6 &13 &24 &43 \\
    \hline
    \# of assertions &    1   &  2     &   4    &   6    &    0   &  0     &  1     &  4     &   0    &   1    &   2    &   4    &   0    &   2    &    3   &  6 & 1& 2& 4 & 9\\
    % \hline
    % Length of call sequence &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \end{tabular}%
    }
  \label{tb:testmethod}
\end{table*}%




% \begin{table}[h!]
% \caption{Test method characteristics. \hl{would be good to collect some of the data by testing level}}
% \centering
% \begin{tabular}{l|c|c|c|c}
% \textbf{Metrics} & \textbf{P25} & \textbf{P50} & \textbf{P75} & \textbf{P90}\\
% \hline
% \hline
% NCLOC & 5 & 9 & 17 & 29\\
% % \hline
% % Cyclomatic Complexity & 1 & 1& 1&2\\
% \hline
% \# of objects created & 0 & 1 & 2 & 4\\
% \hline
% \# of mocks & & & &\\
% \hline
% \# of constructor calls & 0 &  0& 2& 4\\
% \hline
% \# of application calls & & & &\\
% \hline
% \# of library calls &0 & 1&5 &12\\
% \hline
% \# of call-assertion sequence & 1 &2 &4 &8\\
% \hline
% \# of assertions &  & & &\\
% \hline
% Length of assertion sequence &  & & &\\
% \hline
% Length of call sequence & 4 & 9 & 19 & 38\\
% \end{tabular}
% \label{tb:testmethod}
% \end{table}

==> test_quality.tex <==
% \subsection{Coverage Analysis}

% \subsection{Test Characteristics}
% \subsubsection{Bad-path test cases}
% \subsubsection{Order dependent test cases}
